View-Consistent Hierarchical 3D Segmentation Using Ultrametric Feature Fields

Large-scale vision foundation models such as Segment Anything (SAM) demonstrate impressive performance in zero-shot image segmentation at multiple levels of granularity. However, these zero-shot predictions are rarely 3D-consistent. As the camera viewpoint changes in a scene, so do the segmentation predictions, as well as the characterizations of "coarse" or "fine" granularity. In this work, we address the challenging task of lifting multi-granular and view-inconsistent image segmentations into a hierarchical and 3D-consistent representation. We learn a novel feature field within a Neural Radiance Field (NeRF) representing a 3D scene, whose segmentation structure can be revealed at different scales by simply using different thresholds on feature distance. Our key idea is to learn an ultrametric feature space, which unlike a Euclidean space, exhibits transitivity in distance-based grouping, naturally leading to a hierarchical clustering. Put together, our method takes view-inconsistent multi-granularity 2D segmentations as input and produces a hierarchy of 3D-consistent segmentations as output. We evaluate our method and several baselines on synthetic datasets with multi-view images and multi-granular segmentation, showcasing improved accuracy and viewpoint-consistency. We additionally provide qualitative examples of our model's 3D hierarchical segmentations in real world scenes. The code and dataset are available at https://github.com/hardyho/ultrametric_feature_fields

==> sec/bak_0_abstract.tex <==
\begin{abstract}
Recent advances in large-scale 2D segmentation models have significantly improved the quality of zero-shot multi-granularity segmentation. However, achieving consistent 3D segmentation across multiple views in a scene remains a challenging task. Recently, NeRFs have emerged as a popular framework for fusing 3D reconstruction and semantic understanding from 2D data.

In this paper, we propose a novel method that focuses on optimizing a ultrametric feature field within NeRF to achieve hierarchical 3D consistent segmentation, relying solely on view-inconsistent off-the-shelf 2D segmentation as inputs to our method. We introduce a synthetic multi-granularity segmentation dataset to validate the accuracy and view-consistency of our method. Our approach opens up new possibilities for obtaining robust and accurate 3D consistent multi-granularity segmentation derived from view-inconsistent segmentation data.


\end{abstract}

==> sec/bak_1v2_introduction_colton.tex <==
\section{Introduction}
\label{sec:intro}


\begin{itemize}
    \item Large segmentation models, such as SAM\cite{kirillov2023segment}, can handle multi-granularity and arbitrary category segmentation in 2D. The segmentation results and hierarchy are view-inconsistent. \textcolor{red}{Add some failure cases of 10 degrees rotation} 

    \item LeRF\cite{kerr2023lerf} and DFF\cite{kobayashi2022distilledfeaturefields} utilize the feature maps from off-the-shelf 2D image feature extractors and exhibit some segmentation ability in both 2D and 3D. However, the quality of the 2D segmentation generated using these self-supervised 2D image features is notably lower than that of state-of-the-art segmentation models such as SAM trained explicitly for the segmentation task.    

    \item Some methods, such as Semantic-NeRF, train a semantic field in parallel with the RGB field in NeRF and can propagate 3D-consistent semantic labels to novel views with NeRF. However, the segmentation results from SAM have multiple levels of granularity, are not category-specified, and are inconsistent across different views. Semantic-NeRF cannot distill a feature or semantic field from this kind of input.
    
    \item We propose a method capable of generating multi-granularity segmentation results that remain coherent from different views, with view-inconsistent SAM outputs as our supervision. The goal is to aggregate inconsistent and multi-granularity 2D segmentation results from various training views into a single NeRF.

    \item To enable multi-granularity segmentation, we simultaneously train an ultrametric feature field alongside the RGB radiance field. Our model can generate segmentations at varying levels of granularity based on a granularity scalar. The segmentation label of each pixel is unambiguous given a granularity scale, which is different from all euclidean-distance based method.

    \item Our model is trained using 2D off-the-shelf segmentation data that lack consistency in views, hierarchies, and categories. We make no assumptions about the segmentation inputs. To enable training with such data, we introduce a contrastive learning scheme for training the ultrametric feature field.

    \item We perform ultrametric segmentation on a 3D point cloud generated by nerf to produce 3D-consistent segmentation results. 

    \item We introduce a method to enhance NeRF's depth estimation by utilizing SAM output.

    \item We introduce a synthetic multi-granularity segmentation dataset that is based on the Blender dataset to validate the accuracy and view-consistency of our method. We also propose a metric to evaluate the 3D consistency of multi-view 2D segmentation results. 
    
    \item Our method not only surpasses other NeRF-based approaches like DFF and LeRF in terms of accuracy but also achieves accuracy comparable to SAM while yielding significantly more view-consistent results
 
    
\end{itemize}


==> sec/bak_4_experiments.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/seg_maps/image.png}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/seg_maps/gran_2.png}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/seg_maps/gran_1.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/seg_maps/gran_0.png}
    \end{subfigure}
    \caption{\textbf{Blender with Hierarchical Segmentation (Blender-HS)}: We render hierarchical segmentation maps at three levels of granularity, namely \textit{Scene}, \textit{Collection}, and \textit{Object}, using information saved into the blender file by the scene artist.} % for the synthetic dataset with the blender file. }
    \label{fig:seg_maps}

\end{figure}


\section{Experiments}
\label{sec:exp}
We report qualitative and quantitative evaluations for our method and a set of baselines. 
% Firstly, we quantitatively evaluate the quality of multi-granularity segmentation, view-consistency, and segmentation injectivity on a synthetic dataset derived from the Blender Synthetic Datasets~\cite{mildenhall2020nerf}.
In \cref{sec:dataset} we give an overview of the datasets we evaluate on, and we define evaluation metrics that measure segmentation accuracy, view-consistency, and hierarchical consistency. In \cref{sec:comparison} and \cref{sec:ablation}, we present quantitative comparisons and ablation studies. We additionally visualize our method's hierarchical and view-consistent segmentation on real-world scenes from the Tanks and Temples Dataset~\cite{Knapitsch2017}. We present implementation details in \cref{sec:implmentation}.

\subsection{Datasets and Metrics}
\label{sec:dataset}

\todo{Rewrite this paragraph}
To the best of our knowledge, no publicly available dataset contains segmentation labels which are 3D-consistent and hierarchical, and no previous works evaluate on view-consistent and hierarchical segmentation of arbitrary parts and categories. To address this, we introduce a new dataset, and new evaluation metrics, focusing on multi-view and hierarchical segmentation of arbitrary objects.

%To quantitatively evaluate multi-granularity segmentation performance, we require a dataset featuring 3D-consistent annotations for multi-granularity segmentation.
\vspace{-2mm}
\paragraph{Blender with Hierarchical Segmentation}
% To the best of our knowledge, no publicly available dataset exists that captures \textit{both} 3D-consistent and hierarchical segmentation labeling. As consistency and hierarchy are core contributions of our method, 
We create a new synthetic dataset based on the Blender Dataset~\cite{mildenhall2020nerf} which we call Blender with Hierarchical Segmentation (Blender-HS). % Hiearchical and View-Consistent Blender Dataset (Blender-HS). 
% wherein the Blender file is provided, and all objects in the scene are hierarchically organized within the Blender file.
We choose three scenes from the Blender Dataset that exhibit clear hierarchical structure: Lego, Hotdog, and Drums, and for each we define three granularity levels, which we denote as ``scene", ``collection", and ``object". The object level consists of each distinct 3D asset; the ``collection'' level contains 3D asset groupings that were decided by the original artist; the ``scene'' level consists of the entire scene. %The collection level is most interesting, which contains 3D asset groupings that were decided by the original artist. 
%For example, one collection in the Hotdog scene is the hotdog and bun with the ketchup and mustard on top of it. 
While many potential hierarchies exist in general, the artist-defined groupings naturally represent a hierarchy that makes sense for humans.  
\cref{fig:seg_maps} illustrates the ground truth segmentations this process delivers on the Drums scene.
% \colton{@Haodi, we use the artist-defined collections, right?} \haodi{yes}

% We use the \texttt{Separate by Loose Parts} function in Blender to disassemble objects grouped together with \texttt{Mirror} or \texttt{Array} modifiers. We utilize all 100 frames for each scene from the original training split in the Blender Datasets for training, and uniformly sample 10 frames from the original validation split for evaluation. We use \texttt{Segment everything} from SAM to generate 2D segmentation masks for the training data. Additionally, we utilize the ground truth depth map to assess the 3D consistency of segmentation results.

% \begin{itemize}
%     \item There are no datasets that have 3D-consistent multi-granularity segmentation annotations.
%     \item In order to evaluate our method quantitively, we create our datasets from the Blender synthetic datasets from~\cite{mildenhall2020nerf}. We select three of the eight scenes that are organized hierarchically in Blender, specifically the Lego, Hotdog, and Drums scenes. For each of these three scenes, the Blender file includes three levels of granularity: objects, collections, and the foreground scene. We render segmentation maps at different levels of granularity and evaluate our method based on them. 
%     \item \textcolor{red}{We also evaluate our method qualitatively on xx datasets}
    
% \end{itemize}
% \paragraph{Evaluation Metrics}

\vspace{-2mm} 
\noindent\paragraph{PartNet} 
\todo{Add a paragraph here}


\vspace{-2mm} 
\noindent\paragraph{Normalized Covering Score}

To assess the quality of hierarchical segmentation, we use the Normalized Covering (NC) score~\cite{ke2022unsupervised}. This metric averages the Intersection over Union (IoU) between each ground truth mask and the \textit{best-matching} (\ie most-overlapping) predicted mask. 
%Moving forward, we call this the Normalized Covering Score (NC) because hierarchical segmentation lacks a foreground and background. 
We calculate a separate NC score for each granularity and report the mean of these scores. \todo{We also use the metric to evaluate the point cloud segmentation results on PartNet~\cite{Mo_2019_CVPR}}%-granularity NC score.

% The benchmark is defined as \begin{equation}
     % \mathrm {NCovering}(S' \rightarrow  S) = \frac {1}{|S|} \sum \limits _{R \in S} \max \limits _{R' \in S'} \frac {|R \cap R'|}{|R \cup R'|} 
% \end{equation}

% where $S$ denotes all ground truth segmentation masks at the corresponding granularity level, and $S'$ denotes all predicted masks.\\

% \vspace{-5mm} 
\vspace{-2mm} 
\noindent\paragraph{Segmentation Injectivity Score}
In hierarchical segmentation, it is important that each pixel belongs to only one mask for each level of granularity. To measure this, we propose a metric which we call Segmentation Injectivity (SI). 
%
% 
For each ground truth segmentation, we retrieve its {best-matching} predicted mask and sample two random points $p_1$ and $p_2$ from that mask. We then query the model for a new mask at each of these points, at the same granularity. We compute the Intersection over Union (IoU) between the two resulting masks.  %to predict new masks centered about $p_1$ and $p_2$. 
Note that a perfect model will return the same mask at both locations, since these points belong to the same ground-truth segment, whereas a worse model will return masks which may not even overlap. Since the random point sampling introduces some randomness, we run this 100 times per ground truth mask, and average the scores across all ground truth masks and all viewpoints. We find this is more tractable than estimating masks densely, and in practice exhibits low variance. 
%
% \colton{Version 1}
% For each ground truth mask $A_{\text{gt}}$, we identify the \textit{best-matching} predicted mask, $A_{\text{pred}}$, and retrieve the corresponding level of granularity, $t_A$. Next, we sample two random points $p_1$, $p_2$ within $A_{\text{pred}}$ and run segmentation at granularity $t_A$ with input queries $p_1$ and $p_2$, resulting in two newly predicted masks $A_{p_1}$ and $A_{p_2}$. Finally, we compute the Intersection over Union (IoU) between $A_{p_1}$ and $A_{p_2}$. In practice, we run this 100 times per ground truth mask, and average the scores across all ground truth masks and all viewpoints.

% For every ground truth mask, we sample 100 points and calculate the mean Intersection over Union (IoU) to derive the Structural Integrity (SI) score. Following this, we average these scores across all test images within each ground truth granularity level to attain the method's final result.

% We initiate the process by querying the model with a random sampled point within it and identify a granularity level that produce the best-matched mask, denoted as $R$. Subsequently, we randomly select a point within the generated mask and re-query the model with the same granularity level, yielding another mask, denoted as $R'$. We then compute the Intersection over Union (IoU) between $R$ and $R'$: $\frac {|R \cap R'|}{|R \cup R'|}$. 
% For every ground truth mask, we sample 100 points and calculate the mean Intersection over Union (IoU) to derive the Structural Integrity (SI) score. Following this, we average these scores across all test images within each ground truth granularity level to attain the method's final result.
%
%Segmentation Injectivity assesses the disjointedness of segmentation masks at each level of granularity, and a low SI suggests that a point is associated with multiple overlapping masks. Additionally, 
% Note that SI captures an important trade-off with the previously discussed Normalized Covering score
Note there is a trade-off between the SI score and the NC score: predicting an excessive number of overlapping masks could inflate the NC score but would significantly lower the SI score. 



% A hierarchical segmentation satisfies two criteria: (1) each pixel should be assigned to only one mask at a given granularity level, and (2) the boundary of a mask at a higher granularity level circumscribes the boundaries of all contained lower granularity masks. While most hierarchical methods approximately satisfy the second criteria, they struggle to adhere to the first. To address this, we propose a metric to evaluate the first criteria, which we call Segmentation Injectivity (SI).
 
% consistency of model predictions when queried with two distinct points within a mask at the same granularity level. Imperfect SI may result in a point being associated with multiple masks at the same granularity level.
% To evaluate the SI of the model, for each ground truth mask, we initiate the process by querying the model with a random sampled point within it and identify a granularity level that produce the best-matched mask, denoted as $R$. Subsequently, we randomly select a point within the generated mask and re-query the model with the same granularity level, yielding another mask, denoted as $R'$. We then compute the Intersection over Union (IoU) between $R$ and $R'$: $\frac {|R \cap R'|}{|R \cup R'|}$. 
% For every ground truth mask, we sample 100 points and calculate the mean Intersection over Union (IoU) to derive the Structural Integrity (SI) score. Following this, we average these scores across all test images within each ground truth granularity level to attain the method's final result.

\vspace{-2mm} 
\noindent\paragraph{View Consistency Score}

We use a View Consistency (VC) score to measure the 3D consistency of image segmentations. The key idea of this score is to estimate segmentations in two nearby viewpoints independently, and then warp these estimates onto one another, and measure their agreement. %This relies on the fact that under small camera transformations (e.g., moving 10 degrees on the viewing sphere), it is possible to warp masks from one view to another with good accuracy, providing access to ground-truth targets for view-consistency. 
%key idea in this score is to predict two segmentations from camera views that are 10 degrees apart, and measure how well the masks  consistency in mask prediction. 
%Concretely, we begin with a similar process as SI score, and for each ground truth mask $A_{\text{gt}}$ we estimate $A_{\text{pred}}$ and $t_A$. Next, sample point $p_1$ in $A_{\text{pred}}$ and transfer it into new viewpoint 10 degrees off. use ground truth depth and camera parameters to project 
To compute this score, we begin by defining a pixel transformation $T$ from a source viewpoint to another one shifted 10 degrees, using ground truth depth and camera pose.
%we use the ground truth depth and camera parameters from two viewpoints, we can project a pixel in the screen space of one view to the other, denoting the transformation as $f: \mathbb{R}^2 \rightarrow \mathbb{R}^2$. Similarly, we can project a mask from one view to the other, denoted as $f_{mask}: [0, 1]^{H \times W} \rightarrow [0, 1]^{H \times W}$.
Next, for each ground truth segmentation, we retrieve its best-matching predicted mask, sample a random point $p_1$ from that mask, and compute the point's location in the shifted viewpoint $p_2=T(p_1)$. We then obtain segmentation estimates to compare, centered on $p_1$ in the first view and centered on $p_2$ in the second. % first view  then predict a segment centered about $p_1$ in the first image and $p_2$ in the offset image. 
Finally we warp $p_2$'s mask into the $p_1$ viewpoint, and measure IoU with the $p_1$ mask. To ensure that the IoU does not merely reveal occlusion/disocclusion differences, we use ground truth visibility masks to remove pixels which are invisible in either view, before computing the IoU. 
%In all steps, we account for changes in visibility. 
Similar to the other scores, we mitigate noise induced by the random sampling by computing this score 100 times per ground truth mask, and average the scores across all ground truth masks and all viewpoints.
% Additional evaluation details can be found in the supplementary materials.

% We then  to assessing the SI score, we identify $A_{\text{pred}}$ and corresponding threshold $t_A$. Next, we sample point $p_1$ within $A_{\text{pred}}$, and we run segmentation at granularity $t_A$ for the input queries $p_1$ and from another view with $p_2=f(p_1)$, accounting for areas that are not visible in either view. Finally, we compute 
% first query the model with a random sampled point $\textbf{x}$ within the mask and find the given granularity level that produce the best-matched mask $R$. We then query the model from the other view with the point $f(\textbf{x})$ and the same granularity level, removing areas that are not visible in the first view according to the 3D scene, resulting in the mask $R'$.
% the IoU between $A_{p_1}$ and $A_{p_2}$. In practice, we run this 100 times per ground truth mask, and average the scores across all ground truth masks and all viewpoints. Additionally, we set $f_{mask}$ to rotate into a view that offset by 10 degrees. Additional evaluation details can be found in the supplementary materials.

% 
% The View Consistency between two views is defined as:
% \begin{equation}
%     VC(i, j) = \sum_{m_i \in M_i}\frac{1}{|M_i|}mIoU((P_jP_i^Tm_i), m_j)
% \end{equation}
% Where $P_i$ is the camara matrix in the view $i$, and $M_i$ is all segmentation masks in the view $i$. \textcolor{red}{!! Using depth to get the 3d point cloud and project back to 2D in the other view; Segmentation masks in $M_i$ only keep the area that are visible in the other view. Need to improve that formula}

% We set view $j$ to be rotated 10 degrees from view $i$.

\subsection{View-Consistent Hierarchical Segmentation}
\label{sec:comparison}


\begin{table}[tb]
  \caption{\textbf{Results on Blender-HS.} We report Normalized Covering (NC), Segmentation Injectivity (SI), and View Consistency (VC). NC$_\text{obj}$, NC$_\text{coll}$, and NC$_\text{scene}$ refer to the NC score on objects, collections, and scenes, respectively.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    %Heading level & Example & Font size and style\\
    Method & NC$_{obj}$ $\uparrow$ & NC$_{coll}$ $\uparrow$ & NC$_{scene}$ $\uparrow$ & NC$_{mean}$ $\uparrow$ & SI $\uparrow$ & VC $\uparrow$ \\ %\cline{2-5} 
    \midrule
   LSeg~\cite{li2022languagedriven} &0.218&	0.406&	0.670&	0.432 & 0.698 & 0.536\\
   LSeg + DFF~\cite{kobayashi2022distilledfeaturefields} &0.164&	0.427&	0.839	&0.477 & 0.848 & \textbf{0.827}\\
   LeRF~\cite{kerr2023lerf} &0.266 &	0.413	&0.857&	0.512 & 0.598 &0.641  \\
   SAM~\cite{kirillov2023segment} &0.443 &	0.652 &0.787  & 0.627 & 0.808 & 0.462 \\
   SAM3D~\cite{cen2023segment} & 0.460	&0.593	&0.532	&0.528 & - & 0.724 \\
   \hline
   Ours, 2D &\textbf{0.500}	&0.630&	0.940	&0.690 & \textbf{1.000}  & 0.678\\
   Ours &0.480	&\textbf{0.677}&	\textbf{0.971}&	\textbf{0.709} & \textbf{1.000} & 0.789 \\
  \bottomrule
  \end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \footnotesize
    \renewcommand{\arraystretch}{1.3}
    \begin{threeparttable}
        \begin{tabular}{p{2.2cm}|p{1.05cm}<{\centering} p{1.05cm}<{\centering} p{1.05cm}<{\centering}|p{1.05cm}<{\centering}|p{1.05cm}<{\centering}|p{1.05cm}<{\centering}}
            \toprule
           \multirow{2}{*}{Method} & \multicolumn{4}{c|}{NC $\uparrow$} &  \multirow{2}{*}{SI $\uparrow$} & \multirow{2}{*}{VC $\uparrow$} \\ %\cline{2-5} 
            % Method & \multicolumn{4}{|c|}{NC $\uparrow$} &  SI $\uparrow$ & VC $\uparrow$ \\ %\cline{2-5} 
           &NC$_{\text{obj}}$ & NC$_{\text{coll}}$ & NC$_{\text{scene}}$ & NC$_{\text{mean}}$             & & \\
            % Method & NC$_{obj}$ & NC$_{coll}$ & NC$_{scene}$ & NC$_{mean}$ & SI $\uparrow$ & VC $\uparrow$ \\ %\cline{2-5} 
           \midrule
           LSeg~\cite{li2022languagedriven} &0.218&	0.406&	0.670&	0.432 & 0.698 & 0.536\\
           LSeg + DFF~\cite{kobayashi2022distilledfeaturefields} &0.164&	0.427&	0.839	&0.477 & 0.848 & \textbf{0.827}\\
           LeRF~\cite{kerr2023lerf} &0.266 &	0.413	&0.857&	0.512 & 0.598 &0.641  \\
           SAM~\cite{kirillov2023segment} &0.443 &	0.652 &0.787  & 0.627 & 0.808 & 0.462 \\
           SAM3D~\cite{cen2023segment} & 0.460	&0.593	&0.532	&0.528 & - & 0.724 \\
           \hline
           Ours, 2D &\textbf{0.500}	&0.630&	0.940	&0.690 & \textbf{1.000}  & 0.678\\
           Ours &0.480	&\textbf{0.677}&	\textbf{0.971}&	\textbf{0.709} & \textbf{1.000} & 0.789 \\
            \bottomrule
        \end{tabular}
        % \begin{tablenotes}
        %     \footnotesize
        %     \item[\dag] The official code does not perform volume rendering for the feature branch. We implemented volume rendering following the paper, and our implementation outperforms the original codebase.
        % \end{tablenotes}
    \caption{\small{We report Normalized Covering (NC), Segmentation Injectivity (SI), and View Consistency (VC) on our Blender-HS dataset. NC$_\text{obj}$, NC$_\text{coll}$, and NC$_\text{scene}$ refer to the NC score on objects, collections, and scenes, respectively.}}
    \label{tab:comparison}
    \end{threeparttable}
\end{table}
\end{comment}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/lego_feature/image.png}
        \caption{Image}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/lego_feature/dff.png}
        \caption{DFF~\cite{kobayashi2022distilledfeaturefields}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[height=1.0in]{figs/lego_feature/ultra.png}
        \caption{Ours}
    \end{subfigure}
    \caption{\textbf{Feature Visualization}: We visualize rendered feature maps using PCA. The feature map generated by DFF~\cite{kobayashi2022distilledfeaturefields} fails to distinguish between different parts of the Lego. In contrast, our method learns features that can distinguish various Lego bricks.}
    \label{fig:feat-fields}
\end{figure}

\paragraph{Baselines}
%We evaluate our method and a set of baselines on the Blender-HS dataset. % for the task of view-consistent and hierarchical segmentation. 
Because we are the first work to explicitly perform \textit{hierarchical} segmentation in NeRF, we must adapt our baselines to this setting. We adapt language-based methods LSeg~\cite{li2022languagedriven}, DFF~\cite{kobayashi2022distilledfeaturefields}, and LeRF~\cite{kerr2023lerf} to predict a segmentation mask based on a 2D pixel query, by querying the rendered feature map and estimating a segmentation mask via feature similarity. We generate multi-granular predictions by using different thresholds on the feature similarity. % to extract multi-granular predictions. 
% We also adapt SAM3D~\cite{cen2023segment} as a baseline, which we modify to produce multiple segmentations instead of only one: for each ground-truth mask, we sample a pixel within the mask and use SAM3D generate a segmentation across all views, and we repeat this 20 times to generate a variety of masks. 
We also adapt SAM3D~\cite{cen2023segment} as a baseline, which we modify to produce multiple segmentations instead of only one. We propagate SAM outputs from 20 training views into the novel view to generate a variety of masks.
% (also varying the initial viewpoint) to generate a variety of masks. %  for the evaluation. % Because the initial view may influence SAM3D's prediction, we run this across 20 ``initial", views and average the results.
% Note that the SI score does not apply to SAM3D because it has no concept of ``granularity".

\vspace{-2mm}
\paragraph{Quantitative Evaluation}
In Table \ref{tab:comparison}, we report segmentation metrics for our 2D inference mode, our 3D inference mode, and our baselines.  
% For language-driven \red{For LSeg, DFF, and LeRF, as they don't generate any segmentation mask, we randomly select a pixel within the ground-truth mask and query the rendered feature map with different distance thresholds to get masks. For a fair comparison, we adopt a consistent evaluation strategy, employing ultrametric distance in place of the Euclidean distance for our method. For SAM3D, we propagate the segmentation masks from $20$ training views into novel views due to the large time cost (propagating a mask from one view takes around 2 minutes training and it takes around 2 days to propagate all masks from $20$ training views). The NC Score also converge as the number of views fatherly increases. Further details are provided in the supplementary materials.}
 % \red{The SI score does not apply to SAM3D as there's no concept of 'granularity' in SAM3D and we therefore cannot query the model with the same granularity level at the other point.} 
Our method significantly outperforms all other methods in Normalized Covering score (\ie segmentation accuracy). We even outperform SAM, suggesting that our ultrametric feature field not only distills thousands of SAM predictions into a compact set of hierarchical and view-consistent masks, but that our masks are more accurate than \textit{any} of the original SAM predictions.  
Due to the Watershed transform, we also achieve a perfect score on segmentation injectivity (SI), while the other methods (which are non-hierarchical) 
%In contrast all other methods fail to predict non-
tend to predict overlapping masks. Finally, our 3D inference shows significant improvements in view consistency over all methods except DFF. We also point out that 
%DFF's score is perhaps inflated: 
DFF's object-level NC score suggests that it does not segment small objects, which are significantly more challenging to segment in a view-consistent manner, and this fact may inflate the VC score for the method. 

We additionally visualize our ultrametric feature field on the Lego scene in \cref{fig:feat-fields},  showing sharper features than DFF.

\vspace{-2mm}
\paragraph{Qualitative Analysis}
We provide qualitative validation of our method on two real-world scenes from the Tanks and Temples Dataset~\cite{Knapitsch2017}. In \cref{qual-seg-truck}, we visualize three segmentation granularities on the truck scene. In \cref{fig:teaser}, we show our segmentations on the Bobcat tractor scene, which resolves inconsistencies from the source SAM masks. Our method's segmentations tend to have sharp boundaries, and the hierarchical structure decomposes the truck and tractor into intuitive parts and subparts.

\input{sec/partnet_exp}
% suggesting that the hierarchical structure imposed by our method  our method distills multi-view masks   the highest  great view consistency, which is only lower than DFF which is also 3D-consistent, and a perfect hierarchical structure but also outperforms all other methods in the NC score, indicating enhanced segmentation accuracy. \red{The error in the VC score mainly comes from imperfect depth estimation on boundaries and the nearest neighbor querying in 3D.}Notably, our method surpasses SAM, which is used as our supervision during training, suggesting that the feature field aggregates information from multiple views.

\subsection{Ablation Experiments}
\label{sec:ablation}

\begin{table}[tb]
  \caption{Ablation Experiments on Hierarchical Sampling (HS) and Ultrametric Training (UT).
  }
\label{tab:ablation_1}
  \centering
  \begin{tabular}{@{}lcccc@{}}
    \toprule
   {Method} & NC$_{\text{obj}}$ & NC$_{\text{coll}}$ & NC$_{\text{scene}}$ & NC$_{\text{mean}}$ $\uparrow$\\
   \midrule
   Ours & \textbf{0.480}	& \textbf{0.677}	&\textbf{0.971}	&  \textbf{0.709}\\
   % \hline
   w/o UT &0.471	&0.628&	0.964	&0.688\\   
   w/o HS &0.426	&0.640	&0.890	&0.652\\        
  \bottomrule
  \end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \footnotesize
    \renewcommand{\arraystretch}{1.3}
    {
        \begin{tabular}{p{1.6cm}|p{1.3cm}<{\centering} p{1.3cm}<{\centering} p{1.3cm}<{\centering}|p{1.3cm}<{\centering}}
            \toprule
           {method} & NC$_{\text{obj}}$ & NC$_{\text{coll}}$ & NC$_{\text{scene}}$ & NC$_{\text{mean}}$ $\uparrow$\\
           \midrule
           Ours & \textbf{0.480}	& \textbf{0.677}	&\textbf{0.971}	&  \textbf{0.709}\\
           % \hline
           w/o UT &0.471	&0.628&	0.964	&0.688\\   
           w/o HS &0.426	&0.640	&0.890	&0.652\\        
            \bottomrule
        \end{tabular}
       % \vspace{-1mm}
    \caption{\small{Ablation Experiments on Hierarchical Sampling (HS) and Ultrametric Training (UT)}}
    \label{tab:ablation_1}
    }
\end{table}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \footnotesize
    \renewcommand{\arraystretch}{0}
    {
    % \begin{threeparttable}
        \begin{tabular}{p{1.5cm}|p{1.05cm}<{\centering} p{1.05cm}<{\centering} p{1.05cm}<{\centering}|p{1.15cm}<{\centering}|p{1.7cm}<{\centering}}
            \toprule
           {Method} & NC$_{\text{obj}}$ & NC$_{\text{coll}}$ & NC$_{\text{scene}}$ & NC$_{\text{mean}}$ $\uparrow$ & Depth Error $\downarrow$\\
           \midrule
           Ours & \textbf{0.480}	&\textbf{0.677}	&\textbf{0.971}	&\textbf{0.709} & \textbf{0.059}\\
           % \hline
           w/o DC & 0.434	&0.656	&0.923	&0.671 & 0.089\\
            \bottomrule
        \end{tabular}
        % \begin{tablenotes}
        %     \footnotesize
        %     \item[*] The depth error scale adheres to the normalized scene in NeRF.
        % \end{tablenotes}
         % \vspace{-1mm}
        \caption{\small{Ablation Study on Depth Continuity Loss (DC)}}
        \label{tab:ablation_2}
    % \end{threeparttable}
    \vspace{-2mm} 
    }
\end{table}
\end{comment}

\vspace{-4mm}
\noindent\paragraph{Hierarchical Data Sampling}
In \cref{tab:ablation_1} we evaluate the influence of hierarchical data sampling for contrastive learning.
In the baseline approach, positive pairs are randomly sampled within each mask, and negative pairs are sampled with one point inside and one point outside. Results indicate that using the hierarchical sampling strategy improves the overall performance by $5.7$ points.

\vspace{-2mm}
\noindent\paragraph{Ultrametric training}
In \cref{tab:ablation_1} we report the impact of the ultrametric loss, $\ell_{\textrm{ultra}}$. %, into the model training process. 
In the baseline method, we train the feature space using only the Euclidean loss, $\ell_{\textrm{Euclid}}$. %The evaluation process for the baseline method is same as for our approach. 
Results show that the ultrametric training improves the segmentation performance by $2.1$ points.

\vspace{-2mm}
\noindent\paragraph{Depth Continuity Loss}
\cref{tab:ablation_2} shows the influence of using the depth continuity loss during training. In addition to evaluating the NC score, we evaluate depth estimation accuracy, using % between the two experiments and the ground truth depth maps from the synthetic dataset, reporting the 
mean $\ell_2$ error. Incorporating the depth continuity loss improves both segmentation accuracy and depth accuracy. %not only the quality of depth estimation but also enhances . 
\cref{fig:depth continuity} qualitatively illustrates the benefit of the depth continuity loss in real data. %qualitatively motivates using depth continuity in real world data.

\subsection{Implementation Details}
\label{sec:implmentation}

We implement our method using the publicly available codebase from DFF~\cite{kobayashi2022distilledfeaturefields}. %\footnote{\url{https://github.com/pfnet-research/distilled-feature-fields}}
We model our feature branch after the RGB branch of Instant-NGP~\cite{mueller2022instant} -- we employ a multi-resolution grid hash encoder to transform 3D coordinates into features, followed by an MLP. For the grid hash encoder, we configure the number of levels to $17$, features per level to $4$, and the hash map size to $2^{20}$. The MLP comprises three hidden layers with $128$ dimensions each, producing a final output feature of $256$ dimensions. 

On Blender-HS, we train our model for $20,000$ iterations with a batch size of $4096$ and use the same optimization parameters as DFF. In contrastive learning (see \cref{eq:contrastive}), we set the temperature $\tau$ to $0.1$ and sample $64$ positive and negative pairs from each mask. For depth continuity loss, we sample $16$ patches per mask, and begin using the depth continuity loss after $5000$ iterations. 
During 3D inference, we extract a point cloud from training-view depth maps, apply voxel downsampling with voxel size $2\times 10^{-3}$, and run outlier removal with distance threshold $4\times 10^{-3}$ and number threshold of $1$. We build the graph of points using $k_{graph}=16$ nearest neighbors, and we transfer point segmentation labels into a novel view using the mode of $k_{query}=5$ nearest neighbors. We retain $N=200$ graph components and set the distance threshold $d$ to be $5 \times 10^{-3}$. 
Please refer to ~\cref{sec:method} for definitions of the above hyperparameters.

For our quantitative evaluation on Blender-HS, we compute the NC score of LSeg, DFF, LeRF, and our method across 50 distance thresholds ranging from $0.01$ to $0.50$. We follow DFF~\cite{kobayashi2022distilledfeaturefields} and perform all evaluation on $4\times$ downsampled images. For all methods, we exclude masks containing fewer than $20$ pixels. 
% Additionally, we provide qualitative results at a higher resolution.



==> sec/partnet_exp.tex <==
\paragraph{Partnet Experiments}

%# Chair: ['38037', '36717', '40460', '42967', '42213']
%# Table: ['31223', '25622', '21369', '19452', '30878']
%# StorageFurniture: ['45289', '49172', '45869', '48655', '47494']

we conduct experiment on 15 scenes from three categories (chair, table, storage furniture) following the setting of \todo{(!Need Help: where is the rgb data coming from..)} from the test set. Each object is rendered in 24 views and we use 3 of them as test views and the rest as training views. We evaluate the NC score of LSeg+DFF, SAM3D and our method, as these three methods have the best view consistency. We also compare our method against ~\cite{sun2022semantic}, which is a supervised pointcloud segmentation method trained on the trainning set of Partnet~\cite{Mo_2019_CVPR}. We can see that our method can achieve comparable NC score on the finest level. We perform worse on the middle level because our method only generates point clusters that are connected to each other, but some of the ground truth mask are segmented based on the semantic information (e.g. all legs of a chair), which can never be segment as a mask with our method. We don't report the finest level here as it's just the whole object, and it's meaningless in point cloud segmentation task.

There are different numbers of layers in the partnet hierarchical tree for different objects. We split them into three level when we calculate the NC metric: finest, middle, and coarse, where finest is the leaf level and coarse is the root level. 

\begin{table}[tb]
  \caption{\textbf{Results in PartNet.} We report Normalized Covering (NC) on PartNet dataset. NC$_\text{fine}$, NC$_\text{mid}$, and NC$_\text{coar}$ refer to the NC score on three different hierarchy levels.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lcccc@{}}
    \toprule
   {Method} &NC$_{\text{fine}}$ & NC$_{\text{midd}}$ & NC$_{\text{coar}}$ & NC$_{\text{mean}}$ 
    \midrule
   LSeg + DFF~\cite{kobayashi2022distilledfeaturefields} & 0.224 & 0.485 & 0.706& 0.4720 \\
   SAM3D~\cite{cen2023segment} & \textbf{0.510}	&0.608	& 0.668 & 0.596 \\
   \hline
   Ours &0.499&	\textbf{0.633}&	\textbf{0.828} & \textbf{0.653} \\
  \bottomrule
  \end{tabular}
\end{table}

\begin{comment}
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \footnotesize
    \renewcommand{\arraystretch}{1.3}
    \resizebox{0.45\linewidth}{!}
    {
    \begin{threeparttable}
        \begin{tabular}{p{2.2cm}|p{1.05cm}<{\centering} p{1.05cm}<{\centering} p{1.05cm}<{\centering}|p{1.05cm}<{\centering}
            \toprule
           \{Method} &NC$_{\text{fine}}$ & NC$_{\text{midd}}$ & NC$_{\text{coar}}$ & NC$_{\text{mean}}$ 
             \\
            % Method & NC$_{obj}$ & NC$_{coll}$ & NC$_{scene}$ & NC$_{mean}$ & SI $\uparrow$ & VC $\uparrow$ \\ %\cline{2-5} 
           \midrule
          
           LSeg + DFF~\cite{kobayashi2022distilledfeaturefields} & 0.224 & 0.485 & 0.706& 0.4720 \\
           SAM3D~\cite{cen2023segment} & \textbf{0.510}	&0.608	& 0.668 & 0.596 \\
           \hline
           
           Ours &0.499&	\textbf{0.633}&	\textbf{0.828} & \textbf{0.653} \\
            \bottomrule
        \end{tabular}
        % \begin{tablenotes}
        %     \footnotesize
        %     \item[\dag] The official code does not perform volume rendering for the feature branch. We implemented volume rendering following the paper, and our implementation outperforms the original codebase.
        % \end{tablenotes}
    \caption{\small{We report Normalized Covering (NC) on PartNet dataset. NC$_\text{fine}$, NC$_\text{mid}$, and NC$_\text{coar}$ refer to the NC score on three different hierarchy levels.}}
    \label{tab:partnet}
    \end{threeparttable}
    }
\end{table}


\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \footnotesize
    \renewcommand{\arraystretch}{1.3}
    \resizebox{0.45\linewidth}{!}
    {
    \begin{threeparttable}
        \begin{tabular}{p{2.2cm}|p{1.05cm}<{\centering} p{1.05cm}<{\centering} p{1.05cm}<{\centering}|p{1.05cm}<{\centering}
            \toprule
           \{Method} &NC$_{\text{fine}}$ & NC$_{\text{mid}}$ & NC$_{\text{coar}}$ & NC$_{\text{mean}}$ 
             \\
            % Method & NC$_{obj}$ & NC$_{coll}$ & NC$_{scene}$ & NC$_{mean}$ & SI $\uparrow$ & VC $\uparrow$ \\ %\cline{2-5} 
           \midrule
          
           ~\cite{sun2022semantic} & \textbf{0.522} & \textbf{0.750}&	- & \textbf{0.636} \\
           \hline
           
           Ours & 0.489 &	0.604&	 & 0.547
 \\
            \bottomrule
        \end{tabular}
        % \begin{tablenotes}
        %     \footnotesize
        %     \item[\dag] The official code does not perform volume rendering for the feature branch. We implemented volume rendering following the paper, and our implementation outperforms the original codebase.
        % \end{tablenotes}
    \caption{\small{We report Normalized Covering (NC) on PartNet dataset based on point cloud. NC$_\text{fine}$, NC$_\text{mid}$, and NC$_\text{coar}$ refer to the NC score on three different hierarchy levels.}}
    \label{tab:pcd_partnet}
    \end{threeparttable}
    }
\end{table}
\end{comment}


\todo{Noted that SAM3D doesn't produce hierarchical result}



